QuTIE: Quantum optimization for Target Identification by Enzymes

Target Identification by Enzymes (TIE) problem aims to identify the set of enzymes in a given metabolic network, such that their inhibition eliminates a given set of target compounds associated with a disease while incurring minimum damage to the rest of the compounds. This is an NP-complete problem, and thus optimal solutions using classical computers fail to scale to large metabolic networks. In this paper, we consider the TIE problem for identifying drug targets in metabolic networks. We develop the first quantum optimization solution, called QuTIE (Quantum optimization for Target Identification by Enzymes), to this NP-complete problem. We do that by developing an equivalent formulation of the TIE problem in Quadratic Unconstrained Binary Optimization (QUBO) form, then mapping it to a logical graph, which is then embedded on a hardware graph on a quantum computer. Our experimental results on 27 metabolic networks from Escherichia coli, Homo sapiens, and Mus musculus show that QuTIE yields solutions which are optimal or almost optimal. Our experiments also demonstrate that QuTIE can successfully identify enzyme targets already verified in wet-lab experiments for 14 major disease classes.

==> Content/1_prelim.tex <==
%Quantum computing in general and QA in particular are emerging technologies and still not commonly employed in addressing complex computational problems in bioinformatics and computational biology, despite its promise in tackling NP-complete problems more effectively than classical computing methods. 
In this section, we present the fundamental concepts and terminology needed to understand the Quantum Annealing process and how we solve the TIE problem using QA. We first describe the QA workflow for generalized optimization problems. Next, we describe QUBO representation of optimization problems which can be encoded in QA.

\subsection{Quantum annealing and its work flow}

Quantum annealing (QA) is an extension of simulated annealing - a classical optimization method which is effective for solving multi-dimensional optimization problems with large number of local extrema \citep{Finnila1994}. QA works following from the principle that a physical system can be described in term of its energy  via a mathematical description, called \emph{Hamiltonian} function. The Hamiltonian function is a mapping from a state of the system to energy. In a physical system, the state in which the Hamiltonian function returns the lowest energy is called the \emph{ground state} of the system. In QA, we define two quantum systems, described by two different Hamiltonian functions, called \emph{initial Hamiltonian}, and \emph{final Hamiltonian}. Initial Hamiltonian is a function whose ground state happens when all qubits are in a superposition state of 0 and 1. The final Hamiltonian represents the optimization problem we want to solve by QA. QA changes the quantum system described by the initial Hamiltonian, into the quantum system described by the final Hamiltonian. As the quantum systems change, they remain in their ground states. Because the system described by the final Hamiltonian represents the optimization problem, the ground state at the end is interpreted as the optimal solution of the optimization problem. Thus, the key challenge in QA is to design the final Hamiltonian.

To construct a final Hamiltonian from an optimization problem, and to encode it to Quantum Processing Unit (QPU), the first step is to define the optimization problem in a special form, called \emph{Ising model}, or its equivalent representation, called the QUBO form. We describe this model and form later. The resulting QUBO formulates the final Hamiltonian, which the quantum system evolves to from an initial Hamiltonian. We encode the resulting QUBO with a graph called logical graph, and embed the logical graph into a QPU whose topology is called hardware graph. 
We refer the interested reader to~\citep{Choi2008} for detailed description of how logical graph is mapped to hardware graph for QA.
To ensure that the optimal solution of QUBO encoded by the resulting embedding is identical to that encoded by the logical graph, we assign appropriate weights for nodes and edges included in the embedding. Finally, after running the annealing process repeatedly on the QPU, we decode the resulting ground state of the final Hamiltonian with the lowest energy to obtain the final solution for the optimization problem.


\subsection{Ising model, and QUBO formulation}
\label{sec:prelim:formulation}
%\tk{Hoang. This section is not well structured or well written. Expand it a little and step by step define the terms and formulation clearly. I cannot fix it in  this form.}

The Ising model uses variables, which take discrete variables modeling dipole magnet of spin states with values in $\{-1, 1\}$ as the basis. 
It expresses a known NP complete problem, called Ising spin glasses problem in decision form~\citep{Lucas2014}. Given $N$ spins with external magnetic field of the $i^{th}$ spins denoted by $h_i$, and coupling strength between the $i^{th}$ and $j^{th}$ spins denoted by $J_{ij}$, the objective is to decide the state of the $i^{th}$ spin denoted by variables $s_i \in \{-1, 1\}$, such that total energy of the system is minimized. Based on above definition of Ising, for $\mathbf{s} = [s_0, s_1, ..., s_{N}]$, we express the given optimization problem in Ising form as follows: 
\begin{equation} \label{eq:ising}
    H_{\textrm{Ising}}(\mathbf{s}) = -\sum_{i=1}^{N} h_is_i - \sum_{i=1}^{N}\sum_{j=i+1}^{N} J_{i,j}s_is_j
\end{equation}

The Ising model deals with inputs belonging $\{-1, 1\}$ basis. By setting $s_i = 2x_i-1$, we obtain an equivalent function $f(x)$ which works on binary basis. In detail, we have:
\begin{equation} \label{eq:ising_to_qubo}
    f(\mathbf{x}) = -\sum_{i=1}^{N} (a_i-2b_i)x_i - \sum_{i=1}^{N}\sum_{j=i+1}^{N} 4J_{i,j}x_ix_j
\end{equation}
with the constants $a_i = \sum^{N}_{j=i+1} 2J_{i,j} +2h_i$, $b_i = \sum^{N}_{j=i+1} J_{j,i}$. In addition, because binary variable $x$ satisfies $x = x^2$, we replace the first term in the Equation~(\ref{eq:ising_to_qubo}) with $\sum_{i=1}^{N} (a_i-2b_i)x_i^2$, and thus transform the Equation~(\ref{eq:ising_to_qubo}) in following form:
\begin{equation} \label{eq:qubo}
    f(\mathbf{x}) = \sum_{i \leq j}^{N} Q_{i,j}x_ix_j
\end{equation}
The function $f$ is called QUBO. Similarly, we convert a QUBO equation back to Ising model. To solve optimization problems by QA, we have to represent our problem in form of Ising with $\{-1, 1\}$ basis or QUBO with binary basis. In this paper, we present our problem in form of QUBO. From Equation~(\ref{eq:qubo}), we express the state with lowest energy of the final Hamiltonian denoted with $\mathbf{x}^{\ast}$ as 
\begin{equation}
    \mathbf{x}^{\ast} = \textrm{argmin}_{\mathbf{x} \in \{0,1\}^N} f(\mathbf{x})
\end{equation} 


==> Content/4_conclusion.tex <==
In this work, we propose QuTIE, a quantum computing approach for the TIE problem. In our method, we introduce an effective way to represent the TIE problem in form of Quadratic Unconstrained Binary Optimization (QUBO). We set up our experiment with 27 datasets from three different species. We evaluate QuTIE's performance using randomly distributed target compounds, and actual disease-related compounds. In cases of randomly distributed target compounds, we compare QuTIE to one exact method, represented by \emph{OPMET} in cases of small datasets, and one heuristic method represented by \emph{Double-iterative} in cases of large datasets. The experimental results show that QuTIE can provide optimal, or near optimal solutions in small cases while QuTIE outperforms the heuristic method in large cases. In addition, in cases of actual disease-related target compounds, we analyse how the solutions found by QuTIE have impacts on different disease classes. In the future, we plan to expand the TIE problem with more constraints, and adapt our current approach with the power of quantum computing to those expanded problems.

==> Content/name.tex <==

\setcounter{table}{0}
\setcounter{figure}{0} 
\renewcommand{\thetable}{SM. \arabic{table}}
\renewcommand{\thefigure}{SM. \arabic{figure}}


\onecolumn

\pagebreak
\pagestyle{empty}
\section*{{\Large Supplementary Materials 1}}
\section{SM 1: Literature on the TIE problem and limitations}

\begin{figure*}[h]
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=1\textwidth]{plot/hypo_img_1.jpeg}
  \caption{}
  \label{fig:sfig1}
\end{subfigure}
\hfill
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=1\columnwidth]{plot/hypo_img_2.jpeg}
  \caption{}
  \label{fig:sfig2}
\end{subfigure}
\hfill
\begin{subfigure}{.3\textwidth}
  \centering
  \includegraphics[width=1\columnwidth]{plot/hypo_img_3.jpeg}
  \caption{}
  \label{fig:sfig3}
\end{subfigure}

\caption{(a) A metabolic network with a set of enzymes (triangle), reactions (square), and compounds (circle). The target compound is \emph{C3} represented by a double circle. (b) The state of the metabolic network after inhibiting enzyme \emph{E4}. Inhibited nodes are marked by dot-line. Unintentionally inhibited compounds are colored by red. (c) The state of the metabolic network after inhibiting \emph{E1}, and \emph{E2}. }
\label{fig:hypo_img_final}
\end{figure*}

Figure~\ref{fig:hypo_img_final} illustrates an example of the TIE problem. Consider a metabolic network with three enzymes, five reactions and six compounds illustrated in Figure~\ref{fig:sfig1}, our target is to find a set of enzymes such that whose inhibition leads to the elimination of the target compound $C3$ with the least damage. In the Figure~\ref{fig:sfig2}, the inhibition of $E4$ leads to the elimination of $C3$, $C4$, $C5$, and $C6$. Because $C4$, $C5$, and $C6$ are non-target compounds, the damage to the network by inhibiting $E4$ is 3. This selection of inhibited enzymes is not optimal in term of damage. Let's consider another case in which the selection of inhibited enzymes can lead to the optimal damage. If we inhibit the enzymes $E1$ and $E2$, $C1$ is the only non-target compound which is eliminated (see Figure~\ref{fig:sfig3}). Thus, the damage of this enzyme inhibition is 1.

The \emph{OPMET} algorithm solves this problem optimally and improves on the exhaustive search by using branch-and-bound~\citep{}. However, in the worst case, the complexity of OPMET remains exponential in the number of enzymes in the metabolic network. \emph{Double Iterative} method provides a fast heuristic solution in two phases: \emph{Iterative Phase}, and \emph{Fusion Phase}~\citep{}. Iterative Phase finds solutions by tracing the network upstream starting from the target compounds. This phase provides feasible solutions quickly, however these solutions might not be optimal (i.e., although their inhibition stops the production of all the target compounds, but they may yield large damage). Fusion Phase takes these solutions,  and then extends the set of enzymes inferred from them by including neighboring enzymes. It then exhaustively searches for optimal solutions in the extended set. This method has two drawbacks. First, the running time of the second phase is exponential in the number of enzymes in the extended set. Second, if the solutions resulting from the Iterative Phase are not diverse enough, the refined solution can be trapped in a local optima. \emph{Minimum Reaction Cuts (BN-ReactionCut)} problem is similar to the TIE problem~\citep{}. Here, the objective is to find the optimal set of reactions such that their inhibition eliminates a given set of target compounds. Tamura et. al, developed an integer programming (IP) for this problem. This solution however ignores the fact that an enzyme can catalyse multiple reactions. As a result, its solutions can yield high damage values to the TIE problem.

\section{SM 2: Background on Quantum Annealing}
%Quantum computing in general and QA in particular are emerging technologies and still not commonly employed in addressing complex computational problems in bioinformatics and computational biology, despite its promise in tackling NP-complete problems more effectively than classical computing methods. 
In this section, we present the fundamental concepts and terminology needed to understand the Quantum Annealing process and how we solve the TIE problem using QA. We first describe the QA workflow for generalized optimization problems. Next, we describe QUBO representation of optimization problems which can be encoded in QA.


\subsection{Quantum annealing and its work flow}

Quantum annealing (QA) is an extension of simulated annealing - a classical optimization method which is effective for solving multi-dimensional optimization problems with large number of local extrema \citep{}. QA works following from the principle that a physical system can be described in term of its energy  via a mathematical description, called \emph{Hamiltonian} function. The Hamiltonian function is a mapping from a state of the system to energy. In a physical system, the state in which the Hamiltonian function returns the lowest energy is called the \emph{ground state} of the system. In QA, we define two quantum systems, described by two different Hamiltonian functions, called \emph{initial Hamiltonian}, and \emph{final Hamiltonian}. Initial Hamiltonian is a function whose ground state happens when all qubits are in a superposition state of 0 and 1. The final Hamiltonian represents the optimization problem we want to solve by QA. QA changes the quantum system described by the initial Hamiltonian, into the quantum system described by the final Hamiltonian. As the quantum systems change, they remain in their ground states. Because the system described by the final Hamiltonian represents the optimization problem, the ground state at the end is interpreted as the optimal solution of the optimization problem. Thus, the key challenge in QA is to design the final Hamiltonian.

To construct a final Hamiltonian from an optimization problem, and to encode it to Quantum Processing Unit (QPU), the first step is to define the optimization problem in a special form, called \emph{Ising model}, or its equivalent representation, called the QUBO form. We describe this model and form later. The resulting QUBO formulates the final Hamiltonian, which the quantum system evolves to from an initial Hamiltonian. We encode the resulting QUBO with a graph called logical graph, and embed the logical graph into a QPU whose topology is called hardware graph. 
We refer the interested reader to~\citep{} for detailed description of how logical graph is mapped to hardware graph for QA.
To ensure that the optimal solution of QUBO encoded by the resulting embedding is identical to that encoded by the logical graph, we assign appropriate weights for nodes and edges included in the embedding. Finally, after running the annealing process repeatedly on the QPU, we decode the resulting ground state of the final Hamiltonian with the lowest energy to obtain the final solution for the optimization problem.


\subsection{Ising model, and QUBO formulation}
\label{sec:prelim:formulation}
%\tk{Hoang. This section is not well structured or well written. Expand it a little and step by step define the terms and formulation clearly. I cannot fix it in  this form.}

The Ising model uses variables, which take discrete variables modeling dipole magnet of spin states with values in $\{-1, 1\}$ as the basis. 
It expresses a known NP complete problem, called Ising spin glasses problem in decision form~\citep{}. Given $N$ spins with external magnetic field of the $i^{th}$ spins denoted by $h_i$, and coupling strength between the $i^{th}$ and $j^{th}$ spins denoted by $J_{ij}$, the objective is to decide the state of the $i^{th}$ spin denoted by variables $s_i \in \{-1, 1\}$, such that total energy of the system is minimized. Based on above definition of Ising, for $\mathbf{s} = [s_0, s_1, ..., s_{N}]$, we express the given optimization problem in Ising form as follows: 
\begin{equation} \label{eq:ising}
    H_{\textrm{Ising}}(\mathbf{s}) = -\sum_{i=1}^{N} h_is_i - \sum_{i=1}^{N}\sum_{j=i+1}^{N} J_{i,j}s_is_j
\end{equation}

The Ising model deals with inputs belonging $\{-1, 1\}$ basis. By setting $s_i = 2x_i-1$, we obtain an equivalent function $f(x)$ which works on binary basis. In detail, we have:
\begin{equation} \label{eq:ising_to_qubo}
    f(\mathbf{x}) = -\sum_{i=1}^{N} (a_i-2b_i)x_i - \sum_{i=1}^{N}\sum_{j=i+1}^{N} 4J_{i,j}x_ix_j
\end{equation}
with the constants $a_i = \sum^{N}_{j=i+1} 2J_{i,j} +2h_i$, $b_i = \sum^{N}_{j=i+1} J_{j,i}$. In addition, because binary variable $x$ satisfies $x = x^2$, we replace the first term in the Equation~(\ref{eq:ising_to_qubo}) with $\sum_{i=1}^{N} (a_i-2b_i)x_i^2$, and thus transform the Equation~(\ref{eq:ising_to_qubo}) in following form:
\begin{equation} \label{eq:qubo}
    f(\mathbf{x}) = \sum_{i \leq j}^{N} Q_{i,j}x_ix_j
\end{equation}
The function $f$ is called QUBO. Similarly, we convert a QUBO equation back to Ising model. To solve optimization problems by QA, we have to represent our problem in form of Ising with $\{-1, 1\}$ basis or QUBO with binary basis. In this paper, we present our problem in form of QUBO. From Equation~(\ref{eq:qubo}), we express the state with lowest energy of the final Hamiltonian denoted with $\mathbf{x}^{\ast}$ as 
\begin{equation}
    \mathbf{x}^{\ast} = \textrm{argmin}_{\mathbf{x} \in \{0,1\}^N} f(\mathbf{x})
\end{equation} 




\subsection{Quantum Hybrid Framework.} 
In order to exploit full potential of quantum computing, as well as available capability of classical computing, we utilize a framework which combines both classical, and quantum computing, called \emph{Quantum Hybrid Framework}. Basically, the hybrid framework includes three main parts: decomposer, sampler, and composer. Decompsers are built based on classical techniques which aims to split the initial problem into smaller parts. For example, one of the techniques used for decompsers, called \emph{Energy-Impact decomposing} breaks down the initial problem into sub-problems such that results from sub-problems contribute energy to the initial problem's result as much as possible. The second part in the framework are samplers, which are pure Quantum Solvers. The role of samplers is to solve resulting sub-problems splitted by decomposers. Because size of sub-problems is much smaller than the initial problem, samplers can provide results efficiently in a small running time. \hl{In addition, we can apply the fast Hamiltonian reduction to reduce the number of qubits needed to embed the given problems into QPU~\mbox{}, facilitating this process}. The final part is composers which aim to achieve the final result of the initial problem by combining results of sub-problems. We use Quantum Hybrid Framework provided by D-Wave to solve the QUBO formulation we derive in Section~\ref{sec:qubo:form}.
The framework provides us a solution for our QUBO in a pre-set running time. We then infer the QUBO's solution to a corresponding TIE's solution to evaluate the damage. The Framework also provides us the \emph{total running time} which includes total time needed for the framework to find solutions such as programming time, readout time, anneal time, and delay time. Because the actual running time spent on QPU is not separated from the total running time, we can only estimate how much time quantum computing costs to produce solutions by the total running time.


\newpage
\section{SM 3: Dataset description}

\begin{table}[t] 
    \centering
    \captionsetup{justification=centering}
    \caption{Small networks: Metabolic networks from KEGG database grouped by species. $E$, $R$, $C$, Ed  shows the number of enzymes, reactions, compounds, and edges  respectively. 
    %\tk{I don't think we ever use Id in the paper. Remove from Tables 1 and 2}
    }
    \label{table:data_small}
    \begin{tabular}{ |l|l|l|l|l|l| } 
      \hline
      Species & Functions & $E$ & $R$ & $C$ & Ed \\
     \hline
     &Glycerolipid&14&11&10&37\\
&Citrate Cycle&21&19&20&105\\
{\em E.Coli}&Pentose Phosphate&30&27&23&138\\
&Galactose&30&29&31&149\\
&Glycine,serine, and threonine&35&29&29&122\\ \hline

&Glycerolipid&19&18&13&66\\
&Citrate Cycle&23&21&19&115\\
{\em H.Sapiens}&Pentose Phosphate&24&23&20&119\\
&Galactose&23&21&25&121\\
&Pyruvate&31&25&22&118\\ \hline 
&Glycerolipid&19&18&13&66\\
&Citrate Cycle&23&21&19&115\\
{\em M.Musculus}&Pentose Phosphate&24&23&20&119\\
&Galactose&23&21&25&121\\
&Pyruvate&31&25&22&118\\
     \hline
    \end{tabular}
\end{table}

\begin{table}[t]
    \centering
    \captionsetup{justification=centering}
    \caption{Large networks: Metabolic networks from KEGG database grouped by species. $E$, $R$, $C$, Ed  shows the number of enzymes, reactions, compounds, and edges  respectively.}
    \label{table:data_large}
    \begin{adjustbox}{width=0.5\textwidth}
    \begin{tabular}{ |l|l|l|l|l|l| } 
      \hline
      Species & Functions & E & R & C & Ed \\
     \hline
             &Purine&69&89&66&369\\
{\em E.Coli}&Carbon metabolism&78&65&51&292\\
&Nucleotide metabolism&58&97&55&390\\
&Biosynthesis of amino acids&106&101&98&371\\ \hline
&Purine&75&91&62&391\\
{\em H.Sapiens}&Carbon metabolism&71&59&51&246\\
&Nucleotide metabolism&65&96&53&403\\
&Biosynthesis of amino acids&51&46&49&193\\ \hline
&Purine&77&93&64&398\\
{\em M.Musculus}&Carbon metabolism&71&59&51&246\\
&Nucleotide metabolism&65&96&53&403\\
&Biosynthesis of amino acids&53&47&50&200\\
     \ignoreme{
     eco\_L0&&Purine&69&89&66&369\\
eco\_L1&{\em E.Coli}&Carbon metabolism&78&65&51&292\\
eco\_L2&&Nucleotide metabolism&58&97&55&390\\
eco\_L3&&Biosynthesis of amino acids&106&101&98&371\\ \hline
hsa\_L0&&Purine&75&91&62&391\\
hsa\_L1&{\em H.Sapiens}&Carbon metabolism&71&59&51&246\\
hsa\_L2&&Nucleotide metabolism&65&96&53&403\\
hsa\_L3&&Biosynthesis of amino acids&51&46&49&193\\ \hline
mmu\_L0&&Purine&77&93&64&398\\
mmu\_L1&{\em M.Musculus}&Carbon metabolism&71&59&51&246\\
mmu\_L2&&Nucleotide metabolism&65&96&53&403\\
mmu\_L3&&Biosynthesis of amino acids&53&47&50&200\\
}
     \hline
    \end{tabular}
    \end{adjustbox}
\end{table}
We use metabolic pathways for three species: Escherichia coli (\emph{eco} or {\em E.Coli}), Homo sapiens (\emph{hsa} or {\em H.Sapiens}), and Mus musculus (\emph{mmu} or {\em M.Musculus}) from the KEGG database \citep{}. Individual metabolic pathway attaches to a specific function of the species. We categorize these metabolic networks into two groups based on the number of interactions in each: small  and large pathways. 
Tables~\ref{table:data_small} and~\ref{table:data_large} list the networks' characteristics.
%\tk{you need to describe how you select target compounds too} 


\section{SM 4: Correctness of the QuTIE algorithm}

\begin{lemma}
    Let us denote the set of nodes corresponding to each compound in the given metabolic network with $C$, and the inhibition state of each compound $c \in C$ with $x_c$ as explained in Equation~(\ref{eq:indicator:function}). $H_{\text{damage}}$ function in Equation~(\ref{eq:main1}) returns the damage incurred by the states $x_c$ of all the compounds in $C$, multiplied by constant $k_1$.
    \label{lemma:damage}
\end{lemma}

\begin{proof}
From the definition of the variables, $x_c = 1$ only if the compound corresponding to $c$ is inhibited (see Equation~(\ref{eq:indicator:function})). Thus the summation   
$$\sum_{c \in C-C_{\text{target}}} x_c$$ computes the number of inhibited compounds which are not targeted, and thus, it is equal to the damage incurred on the given network. Therefore, Equation~(\ref{eq:main1}) returns the damage incurred by the states $x_c$ of all the compounds in $C$, multiplied by constant $k_1$.
\end{proof}

\begin{lemma}
    Let us denote the set of nodes corresponding to each compound in the given metabolic network with $C$, and the inhibition state of each compound $c \in C$ with $x_c$ as explained in Equation~(\ref{eq:indicator:function}). $H_{\text{target}}$ function in Equation~(\ref{eq:main2}) returns the number of target compounds which are not inhibited by the states $x_c$ of all the compounds in $C$, multiplied by constant $k_2$.
    \label{lemma:target}
\end{lemma}

\begin{proof}
From the definition of the variables, $x_c = 1$ only if the compound corresponding to $c$ is inhibited (see Equation~(\ref{eq:indicator:function})). Each term $(1 - x_c)$ returns 1 if the compound corresponding to $c$ is not inhibited (i.e., $x_c = 0$). It returns 0 otherwise.
Thus the summation   $$\sum_{c \in C_{\text{target}}} (1 - x_c)$$
computes the number of target compounds which fail to be inhibited. Therefore, Equation~(\ref{eq:main2}) returns the number of target compounds which are not inhibited by the states $x_c$ of all the compounds in $C$, multiplied by constant $k_2$.
\end{proof}

\begin{lemma}
    Let us denote the set of nodes in the given metabolic network with $V_G$, and the inhibition state of each entity (compound, reaction, or enzyme) $u \in V_G$ with $x_u$ as explained in Equation~(\ref{eq:indicator:function}). Let us denote the set of nodes corresponding to each reaction with $R$. In addition, we define the set of neighbors of a node $r \in R$ as $N(r)$, and auxiliary binary variables
    $t_{r\alpha}$ with $0 \leq \alpha \leq |N(r)|$ which is equal to 1 if $x_r - \sum_{v \in N(r)} x_{v} + \alpha = 0$, and equal to 0 if otherwise. $H_{\text{reaction}}$ function in Equation~(\ref{eq:main3}) returns 0 only if all the reactions satisfy the inhibition conditions provided in Equation~(\ref{eq:sub1}) by the states as given in $x_u$, $\forall u \in V_G$ and auxiliary binary variables $t_{r\alpha}$ with $r \in R$ and $0 \leq \alpha \leq N(r)$. Otherwise, it returns a positive number.
    \label{lemma:reaction}
\end{lemma}

\begin{proof}
For each node $r \in R$, the inhibition condition provided in Equation~(\ref{eq:sub1}) can be presented by two Inequalities (\ref{eq:sub2}) and (\ref{eq:sub3}). Specifically, the variables $x_r$ with $r \in R$ and $x_v$ with $v \in N(r)$ satisfies Equation~(\ref{eq:sub1}) if and only if they satisfies two Inequalities (\ref{eq:sub2}) and \ref{eq:sub3}.

Let us consider the Inequality~(\ref{eq:sub2}) $$x_r \geq x_v \forall v \in N(r)$$ 
Given that the value of $x_u$ with $u \in V_G$ only receives the value of 0 and 1, Inequality~(\ref{eq:sub2}) holds if and only if $x_r - x_v = 0$ or $x_r - x_v - 1 = 0$ which is equivalent to $(x_r - x_v)^2 + (x_r - x_v - 1)^2 = 1$ for all $r \in R$. In general, Inequality~(\ref{eq:sub2}) holds if and only if Expression 
\begin{equation}\label{eq:suppl:reaction:express:1}
    \sum_{v \in N(r)}[(x_r - x_{v})^2 + (x_r - x_{v} - 1)^2] - |N(r)|
\end{equation} returns the value of 0. Otherwise, the above Expression returns a positive number \textbf{(a)}.

Next, let us consider the Inequality~(\ref{eq:sub3}) $$0 \geq x_r - \sum_{v \in N(r)} x_{v}$$

We denote the difference $x_r - \sum_{v \in N(r)} x_{v}$ as $d_r$ for all $r \in R$. We observe that Inequality~(\ref{eq:sub3}) holds if and only if $d_r \leq 0$. Given that the value of $x_u$ with $u \in V_G$ only receives the value of 0 and 1, the valid values of $d_r$ which satisfy Inequality~(\ref{eq:sub3}) are from $-|N(r)|$ to 0. We have that the auxiliary variable $t_{r\alpha} = 1$ if and only if $d_r + \alpha = 0$ for all $r \in R$. It is equivalent to two Equations as follows:
\begin{equation}\label{eq:suppl:reaction:equation:1}
    x_r - \sum_{v \in N(r)}x_{v} + \sum_{\alpha=0}^{|N(r)|}(\alpha t_{r\alpha}) = 0 \forall r \in R
\end{equation}

\begin{equation}\label{eq:suppl:reaction:equation:2}
    1 - \sum_{\alpha=0}^{|N(r)|} t_{r\alpha} = 0 \forall r \in R
\end{equation}

As a result, Inequality~(\ref{eq:sub3}) holds if and only if Equations~(\ref{eq:suppl:reaction:equation:1}) and Equation~(\ref{eq:suppl:reaction:equation:2}) hold for all $r \in R$. In general, for each $r\in R$, Inequality~(\ref{eq:sub3}) holds if and only if Expression 
\begin{equation}\label{eq:suppl:reaction:express:2}
    \Biggr[x_r - \sum_{v \in N(r)}x_{v} + \sum_{\alpha=0}^{|N(r)|}(\alpha t_{r\alpha}) \Biggr]^2 + (1-\sum_{\alpha=0}^{|N(r)|}t_{r\alpha})^2
\end{equation} returns 0. Otherwise, the above Expression returns a positive number \textbf{(b)}.

By summing up Expression~(\ref{eq:suppl:reaction:express:1}) and (\ref{eq:suppl:reaction:express:2}) for all $r \in R$, we can obtain $H_{\text{reaction}}$. Based on statements \textbf{(a)} and \textbf{(b)}, we can conclude that $H_{\text{reaction}}$ function in Equation~(\ref{eq:main3}) returns 0 only if all the reactions satisfy the inhibition conditions provided in Equation~(\ref{eq:sub1}) by the states as given in $x_u$, $\forall u \in V_G$ and auxiliary binary variables $t_{r\alpha}$ with $r \in R$ and $0 \leq \alpha \leq N(r)$. Otherwise, it returns a positive number.
\end{proof}

\begin{lemma}
    Let us denote the set of nodes in the given metabolic network with $V_G$, and the inhibition state of each entity (compound, reaction, or enzyme) $u \in V_G$ with $x_u$ as explained in Equation~(\ref{eq:indicator:function}). Let us denote the set of nodes corresponding to each compound with $C$. In addition, we define the set of neighbors of a node $c \in C$ as $N(c)$, and auxiliary binary variables
    $w_{c\beta}$ with $0 \leq \beta \leq |N(c)|$ which which is equal to 1 if $x_c - \sum_{v \in N(c)}x_{v} - 1 + \beta = 0$, and equal to 0 if otherwise. $H_{\text{compound}}$  function in Equation~(\ref{eq:main4}) returns 0 only if all the compounds satisfy the inhibition conditions provided in Equation~(\ref{eq:sub6}) by the states as given in $x_u$, $\forall u \in V_G$ and auxiliary binary variables $w_{c\beta}$ with $c \in C$ and $0 \leq \beta \leq N(c)$. Otherwise, it returns a positive number.
    \label{lemma:compound}
\end{lemma}

\begin{proof}
For each node $c \in C$, the inhibition condition provided in Equation~(\ref{eq:sub6}) can be presented by two Inequalities (\ref{eq:sub7}) and (\ref{eq:sub8}). Specifically, the variables $x_c$ with $c \in C$ and $x_v$ with $v \in N(c)$ satisfies Equation~(\ref{eq:sub6}) if and only if they satisfies two Inequalities (\ref{eq:sub7}) and (\ref{eq:sub8}).

Let us consider the Inequality~(\ref{eq:sub7}) $$x_c \leq x_{v}\forall v \in N(c)$$
Given that the value of $x_u$ with $u \in V_G$ only receives the value of 0 and 1, Inequality~(\ref{eq:sub7}) holds if and only if $x_c - x_v = 0$ or $x_c - x_v + 1 = 0$ which is equivalent to $(x_c - x_v)^2 + (x_c - x_v + 1)^2 = 1$ for all $c \in C$. In general, Inequality~(\ref{eq:sub7}) holds if and only if Expression 
\begin{equation}\label{eq:suppl:compound:express:1}
    \sum_{v \in N(c)}[(x_c - x_{v})^2 + (x_c - x_{v} + 1)^2] - |N(c)|
\end{equation} returns the value of 0. Otherwise, the above Expression returns a positive number \textbf{(a)}.

Next, let us consider the Inequality~(\ref{eq:sub8}) $$-|N(c)| \leq x_c - \sum_{v \in N(c)}x_{v} - 1$$

We denote the difference $x_c - \sum_{v \in N(c)} x_{v} - 1$ as $d_c$ for all $c \in C$. We observe that Inequality~(\ref{eq:sub8}) holds if and only if $-|N(c)| \leq d_c$. Given that the value of $x_u$ with $u \in V_G$ only receives the value of 0 and 1, the valid values of $d_c$ which satisfy Inequality~(\ref{eq:sub8}) are from $-|N(r)|$ to 0. We have that the auxiliary variable $w_{c\beta} = 1$ if and only if $d_c + \beta = 0$ for all $c \in C$. It is equivalent to two Equations as follows:
\begin{equation}\label{eq:suppl:compound:equation:1}
    x_c - \sum_{v \in N(c)}x_{v} - 1 + \sum_{\beta=0}^{|N(r)|}(\beta w_{c\beta}) = 0 \forall c \in C
\end{equation}

\begin{equation}\label{eq:suppl:compound:equation:2}
    1 - \sum_{\beta=0}^{|N(c)|} w_{c\beta} = 0 \forall c \in C
\end{equation}

As a result, Inequality~(\ref{eq:sub8}) holds if and only if Equations~(\ref{eq:suppl:compound:equation:1}) and Equation~(\ref{eq:suppl:compound:equation:2}) hold for all $c \in C$. In general, for each $c\in C$, Inequality~(\ref{eq:sub8}) holds if and only if Expression 
\begin{equation}\label{eq:suppl:compound:express:2}
    \Biggl[ x_c - \sum_{v \in N(c)}x_{v}  - 1 + \sum_{\beta=0}^{|N(c)|}(\beta w_{c\beta}) \Biggr]^2 + (1-\sum_{\beta=0}^{|N(c)|}w_{c\beta})^2
\end{equation} returns 0. Otherwise, the above Expression returns a positive number \textbf{(b)}.

By summing up Expression~(\ref{eq:suppl:compound:express:1}) and (\ref{eq:suppl:compound:express:2}) for all $c \in C$, we can obtain $H_{\text{compound}}$. Based on statements \textbf{(a)} and \textbf{(b)}, we can conclude that $H_{\text{compound}}$ function in Equation~(\ref{eq:main3}) returns 0 only if all the compounds satisfy the inhibition conditions provided in Equation~(\ref{eq:sub6}) by the states as given in $x_u$, $\forall u \in V_G$ and auxiliary binary variables $w_{c\beta}$ with $c \in C$ and $0 \leq \beta \leq N(c)$. Otherwise, it returns a positive number.
\end{proof}


\begin{thm}
    Let us denote the set of nodes in the given metabolic network with $V_G$, the inhibition state of each entity (compound, reaction, or enzyme) $u \in V_G$ with $x_u$ as explained in Equation~(\ref{eq:indicator:function}), auxiliary variables $t_{r\alpha}$ with $r \in R, 0 \leq \alpha \leq |N(r)|$, and auxiliary variables $w_{c\beta}$ with $c \in C, 0 \leq \beta \leq |N(c)|$. The values of all the variables $x_u$, $t_{r\alpha}$ and $w_{c\beta}$ which minimize the objective function in Equation~(\ref{eq:objective}) optimally solves the TIE problem.
    \label{theorem:objective}
\end{thm}

\begin{proof}
In  order to prove this theorem, we need to prove two statements: The values of all the variables $x_u$ which minimize the objective function in Equation~(\ref{eq:objective}) satisfy both of the following:
\begin{enumerate}
    \item they are a valid solution (i.e., the given states inhibit all targeted compounds.)
    \item they minimize damage.
\end{enumerate}
The objective function $H$ given in Equation~(\ref{eq:objective}) is the summation of $H_{\text{damage}}$, $H_{\text{target}}$, $H_{\text{reaction}}$ and $H_{\text{compound}}$. From Lemma~\ref{lemma:damage}, \ref{lemma:reaction} and \ref{lemma:compound}, $H_{\text{target}}$, $H_{\text{reaction}}$ and $H_{\text{compound}}$ returns the minimum value of 0 if and only if values of all variables $x_u$, $t_{r\alpha}$ and $w_{c\beta}$ satisfy target inhibition constraint given in Equation~(\ref{eq:sub_add1}) and inhibition conditions given in Equation~(\ref{eq:sub1}) and (\ref{eq:sub6}). Thus, the values of those variables that make the summation of $H_{\text{target}}$, $H_{\text{reaction}}$ and $H_{\text{compound}}$ equal to 0 are a valid solution \textbf{(a)}.

On the other hand, $H_{\text{damage}}$ specifies the damage inferred from the values of those variables. If we set the values of constants $k_2$, $k_3$, and $k_4$ in $H_{\text{target}}$, $H_{\text{reaction}}$ and $H_{\text{compound}}$ respectively big enough such that every positive values of $H_{\text{target}}$, $H_{\text{reaction}}$ and $H_{\text{compound}}$ are bigger than the maximum value of $H_{\text{damage}}$, the value of $H$ for invalid values of variables $x_u$, $t_{r\alpha}$ and $w_{c\beta}$ is always bigger than that for valid values of those variables. In addition, because the values of $H_{\text{target}}$, $H_{\text{reaction}}$ and $H_{\text{compound}}$ for valid values of those variables are all 0, the value of $H$ for valid values of those variables is equal to $H_{\text{damage}}$. Therefore, the values of variables $x_u$, $t_{r\alpha}$ and $w_{c\beta}$ that minimize the objective function $H$ also minimize the damage \textbf{(b)}.

From \textbf{(a)} and \textbf{(b)}, we prove that the values of all the variables $x_u$, $t_{r\alpha}$ and $w_{c\beta}$ which minimize the objective function in Equation~(\ref{eq:objective}) optimally solves the TIE problem.
\end{proof}

==> full-author-bibliography.tex <==

@article{Lu2014,
    author = {Lu, Wei AND Tamura, Takeyuki AND Song, Jiangning AND Akutsu, Tatsuya},
    journal = {PLOS ONE},
    publisher = {Public Library of Science},
    title = {Integer Programming-Based Method for Designing Synthetic Metabolic Networks by Minimum Reaction Insertion in a Boolean Model},
    year = {2014},
    month = {03},
    volume = {9},
    pages = {1-14},
    number = {3},

}

@Article{Li2011,
author={Li, Zhenping
and Wang, Rui-Sheng
and Zhang, Xiang-Sun},
title={Two-stage flux balance analysis of metabolic networks for drug target identification},
journal={BMC Systems Biology},
year={2011},
month={Jun},
day={20},
volume={5},
number={1},
pages={S11}
}


@INPROCEEDINGS {Thai2022,
author = {P. Thai and M. T. Thai and T. Vu and T. N. Dinh},
booktitle = {2022 IEEE International Conference on Quantum Computing and Engineering (QCE)},
title = {FastHare: Fast Hamiltonian Reduction for Large-scale Quantum Annealing},
year = {2022},
volume = {},
issn = {},
pages = {114-124},
address = {Los Alamitos, CA, USA},
month = {sep}
}


@Article{Zielinski2015,
author={Zielinski and et al},
title={Pharmacogenomic and clinical data link non-pharmacokinetic metabolic dysregulation to drug side effect pathogenesis},
journal={Nature Communications},
year={2015},
month={Jun},
day={09},
volume={6},
number={1},
pages={7101},
}

@inbook{Tamura2011,
author = {Tamura, Takeyuki and Takemoto, Kazuhiro and Akutsu, Tatsuya},
year = {2011},
month = {01},
pages = {},
title = {Finding Minimum Reaction Cuts of Metabolic Networks Under a Boolean Model Using Integer Programming and Feedback Vertex Sets}
}

@Article{Choi2008,
author={Choi, Vicky},
title={Minor-embedding in adiabatic quantum computation: I. The parameter setting problem},
journal={Quantum Information Processing},
year={2008},
month={Oct},
day={01},
volume={7},
number={5},
pages={193-209},
}

@article {Mulligan2019,
	author = {Mulligan and et al},
	title = {Designing Peptides on a Quantum Computer},
	elocation-id = {752485},
	year = {2019},
	publisher = {Cold Spring Harbor Laboratory},
	abstract = {Although a wide variety of quantum computers are currently being developed, actual computational results have been largely restricted to contrived, artificial tasks. Finding ways to apply quantum computers to useful, real-world computational tasks remains an active research area. Here we describe our mapping of the protein design problem to the D-Wave quantum annealer. We present a system whereby Rosetta, a state-of-the-art protein design software suite, interfaces with the D-Wave quantum processing unit to find amino acid side chain identities and conformations to stabilize a fixed protein backbone. Our approach, which we call the QPacker, uses a large side-chain rotamer library and the full Rosetta energy function, and in no way reduces the design task to a simpler format. We demonstrate that quantum-annealer-based design can be applied to complex real-world design tasks, producing designed molecules comparable to those produced by widely adopted classical design approaches. We also show through large-scale classical folding simulations that the results produced on the quantum annealer can inform wet-lab experiments. For design tasks that scale exponentially on classical computers, the QPacker achieves nearly constant runtime performance, independent of the complexity of the task, up to the limits of the quantum computer{\textquoteright}s size.This document is a preprint of a scientific manuscript, and the developments that it reports have not been subjected to peer review.},
	journal = {bioRxiv}
}


@article{Preskill2018,
  title = {Quantum {C}omputing in the {NISQ} era and beyond},
  author = {Preskill, John},
  journal = {{Quantum}},
  publisher = {{Verein zur F{\"{o}}rderung des Open Access Publizierens in den Quantenwissenschaften}},
  volume = {2},
  pages = {79},
  month = aug,
  year = {2018}
}

@article{Shor1999,
author = {Shor, Peter W.},
title = {Polynomial-Time Algorithms for Prime Factorization and Discrete Logarithms on a Quantum Computer},
journal = {SIAM Review},
volume = {41},
number = {2},
pages = {303-332},
year = {1999}
}


@article{Kanehisa2000,
    author = {Kanehisa, Minoru and Goto, Susumu},
    title = "{KEGG: Kyoto Encyclopedia of Genes and Genomes}",
    journal = {Nucleic Acids Research},
    volume = {28},
    number = {1},
    pages = {27-30},
    year = {2000},
    month = {01},
    abstract = "{KEGG (Kyoto Encyclopedia of Genes and Genomes) is a knowledge base for systematic analysis of gene functions, linking genomic information with higher order functional information. The genomic information is stored in the GENES database, which is a collection of gene catalogs for all the completely sequenced genomes and some partial genomes with up-to-date annotation of gene functions. The higher order functional information is stored in the PATHWAY database, which contains graphical representations of cellular processes, such as metabolism, membrane transport, signal transduction and cell cycle. The PATHWAY database is supplemented by a set of ortholog group tables for the information about conserved subpathways (pathway motifs), which are often encoded by positionally coupled genes on the chromosome and which are especially useful in predicting gene functions. A third database in KEGG is LIGAND for the information about chemical compounds, enzyme molecules and enzymatic reactions. KEGG provides Java graphics tools for browsing genome maps, comparing two genome maps and manipulating expression maps, as well as computational tools for sequence comparison, graph comparison and path computation. The KEGG databases are daily updated and made freely available (http://www.genome.ad.jp/kegg/ ).}"
}

@incollection{Song2011,
author = {Bin Song and I. Esra Büyüktahtakın and Nirmalya Bandyopadhyay and Sanjay Ranka and Tamer Kahveci},
title = {Identifying Enzyme Knockout Strategies on Multiple Enzyme Associations},
booktitle = {Bioinformatics},
publisher = {IntechOpen},
address = {Rijeka},
year = {2011},
editor = {Mahmood A. Mahdavi},
chapter = {17}
}

@article{Song2009,
author = {Song, Bin and Sridhar, Padmavati and Kahveci, Tamer and Ranka, Sanjay},
title = {Double iterative optimisation for metabolic network-based drug target identification},
journal = {International Journal of Data Mining and Bioinformatics},
volume = {3},
number = {2},
pages = {124-144},
year = {2009}
}

@article{Sridhar2008,
author = {Sridhar, Padmavati and Song, Bin and Kahveci, Tamer and Ranka, Sanjay},
year = {2008},
month = {02},
pages = {291-302},
title = {Mining metabolic network for optimal drug targets},
volume = {13},
journal = {Pacific Symposium on Biocomputing. Pacific Symposium on Biocomputing}
}

@ARTICLE{Carman2008,
  title    = "Phosphatidic acid phosphatase, a key enzyme in the regulation of
              lipid synthesis",
  author   = "Carman, George M and Han, Gil-Soo",
  journal  = "J Biol Chem",
  volume   =  284,
  number   =  5,
  pages    = "2593--2597",
  month    =  sep,
  year     =  2008,
  address  = "United States",
  language = "en"
}

@article{Goodrich2018,
author = {Goodrich, Timothy D. and Sullivan, Blair D. and Humble, Travis S.},
title = {Optimizing Adiabatic Quantum Program Compilation Using a Graph-Theoretic Framework},
year = {2018},
issue_date = {May 2018},
publisher = {Kluwer Academic Publishers},
address = {USA},
volume = {17},
number = {5},
issn = {1570-0755},
url = {https://doi.org/10.1007/s11128-018-1863-4},
doi = {10.1007/s11128-018-1863-4},
abstract = {Adiabatic quantum computing has evolved in recent years from a theoretical field into an immensely practical area, a change partially sparked by D-Wave System's quantum annealing hardware. These multimillion-dollar quantum annealers offer the potential to solve optimization problems millions of times faster than classical heuristics, prompting researchers at Google, NASA and Lockheed Martin to study how these computers can be applied to complex real-world problems such as NASA rover missions. Unfortunately, compiling (embedding) an optimization problem into the annealing hardware is itself a difficult optimization problem and a major bottleneck currently preventing widespread adoption. Additionally, while finding a single embedding is difficult, no generalized method is known for tuning embeddings to use minimal hardware resources. To address these barriers, we introduce a graph-theoretic framework for developing structured embedding algorithms. Using this framework, we introduce a biclique virtual hardware layer to provide a simplified interface to the physical hardware. Additionally, we exploit bipartite structure in quantum programs using odd cycle transversal (OCT) decompositions. By coupling an OCT-based embedding algorithm with new, generalized reduction methods, we develop a new baseline for embedding a wide range of optimization problems into fault-free D-Wave annealing hardware. To encourage the reuse and extension of these techniques, we provide an implementation of the framework and embedding algorithms.},
journal = {Quantum Information Processing},
month = {may},
pages = {1–26},
numpages = {26}
}

@Article{Choi2011,
author={Choi, Vicky},
title={Minor-embedding in adiabatic quantum computation: {II}. Minor-universal graph design},
journal={Quantum Information Processing},
year={2011},
month={Jun},
day={01},
volume={10},
number={3},
pages={343-353},
abstract={In Choi (Quantum Inf Process, 7:193--209, 2008), we introduced the notion of minor-embedding in adiabatic quantum optimization. A minor-embedding of a graph G in a quantum hardware graph U is a subgraph of U such that G can be obtained from it by contracting edges. In this paper, we describe the intertwined adiabatic quantum architecture design problem, which is to construct a hardware graph U that satisfies all known physical constraints and, at the same time, permits an efficient minor-embedding algorithm. We illustrate an optimal complete-graph-minor hardware graph. Given a family {\$}{\$}{\{}{\backslash}mathcal{\{}F{\}}{\}}{\$}{\$}of graphs, a (host) graph U is called {\$}{\$}{\{}{\backslash}mathcal{\{}F{\}}{\}}{\$}{\$}-minor-universal if for each graph G in {\$}{\$}{\{}{\backslash}mathcal{\{}F{\}}, U{\}}{\$}{\$}contains a minor-embedding of G. The problem for designing a {\$}{\$}{\{}{\{}{\backslash}mathcal{\{}F{\}}{\}}{\}}{\$}{\$}-minor-universal hardware graph Usparsein which {\$}{\$}{\{}{\{}{\backslash}mathcal{\{}F{\}}{\}}{\}}{\$}{\$}consists of a family of sparse graphs (e.g., bounded degree graphs) is open.},
issn={1573-1332},
doi={10.1007/s11128-010-0200-3},
url={https://doi.org/10.1007/s11128-010-0200-3}
}

@article{Klymko2012,
author = {Klymko, Christine and Sullivan, Blair and Humble, Travis},
year = {2012},
month = {10},
pages = {},
title = {Adiabatic Quantum Programming: Minor Embedding With Hard Faults},
volume = {13},
journal = {Quantum Information Processing},
doi = {10.1007/s11128-013-0683-9}
}

@misc{Cai2014,
  doi = {10.48550/ARXIV.1406.2741},
  
  url = {https://arxiv.org/abs/1406.2741},
  
  author = {Cai, Jun and Macready, William G. and Roy, Aidan},
  
  keywords = {Quantum Physics (quant-ph), Data Structures and Algorithms (cs.DS), Combinatorics (math.CO), FOS: Physical sciences, FOS: Physical sciences, FOS: Computer and information sciences, FOS: Computer and information sciences, FOS: Mathematics, FOS: Mathematics, 05C83, 81P68},
  
  title = {A practical heuristic for finding graph minors},
  
  publisher = {arXiv},
  
  year = {2014},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@Article{Boothby2016,
author={Boothby, Tomas
and King, Andrew D.
and Roy, Aidan},
title={Fast clique minor generation in Chimera qubit connectivity graphs},
journal={Quantum Information Processing},
year={2016},
month={Jan},
day={01},
volume={15},
number={1},
pages={495-508},
abstract={The current generation of D-Wave quantum annealing processor is designed to minimize the energy of an Ising spin configuration whose pairwise interactions lie on the edges of a Chimera graph {\$}{\$}{\{}{\backslash}mathcal {\{}C{\}}{\}}{\_}{\{}M,N,L{\}}{\$}{\$}. In order to solve an Ising spin problem with arbitrary pairwise interaction structure, the corresponding graph must be minor-embedded into a Chimera graph. We define a combinatorial class of native clique minors in Chimera graphs with vertex images of uniform, near minimal size and provide a polynomial-time algorithm that finds a maximum native clique minor in a given induced subgraph of a Chimera graph. These minors allow improvement over recent work and have immediate practical applications in the field of quantum annealing.},
issn={1573-1332},
doi={10.1007/s11128-015-1150-6},
url={https://doi.org/10.1007/s11128-015-1150-6}
}

@InProceedings{Bernal2020,
author="Bernal and et al",
title="Integer Programming Techniques for Minor-Embedding in Quantum Annealers",
booktitle="Integration of Constraint Programming, Artificial Intelligence, and Operations Research",
year="2020",
pages="112--129",
abstract="A major limitation of current generations of quantum annealers is the sparse connectivity of manufactured qubits in the hardware graph. This technological limitation has generated considerable interest, motivating efforts to design efficient and adroit minor-embedding procedures that bypass sparsity constraints. In this paper, starting from a previous equational formulation by Dridi et al. (arXiv:1810.01440), we propose integer programming (IP) techniques for solving the minor-embedding problem. The first approach involves a direct translation from the previous equational formulation to IP, while the second decomposes the problem into an assignment master problem and fiber condition checking subproblems. The proposed methods are able to detect instance infeasibility and provide bounds on solution quality, capabilities not offered by currently employed heuristic methods. We demonstrate the efficacy of our methods with an extensive computational assessment involving three families of random graphs of varying sizes and densities. The direct translation as a monolithic IP model can be solved with existing commercial solvers yielding valid minor-embeddings but it is outperformed, overall, by the decomposition approach. Our results demonstrate the promise of our methods for the studied benchmarks, highlighting the advantages of using IP technology for minor-embedding problems.",
isbn="978-3-030-58942-4"
}

@article{Serra2022,
author = {Serra and et al},
title = {Template-Based Minor Embedding for Adiabatic Quantum Optimization},
journal = {INFORMS Journal on Computing},
volume = {34},
number = {1},
pages = {427-439},
year = {2022},
doi = {10.1287/ijoc.2021.1065},

URL = { 
        https://doi.org/10.1287/ijoc.2021.1065
    
},
eprint = { 
        https://doi.org/10.1287/ijoc.2021.1065
    
}
,
    abstract = { Quantum annealing (QA) can be used to quickly obtain near-optimal solutions for quadratic unconstrained binary optimization (QUBO) problems. In QA hardware, each decision variable of a QUBO should be mapped to one or more adjacent qubits in such a way that pairs of variables defining a quadratic term in the objective function are mapped to some pair of adjacent qubits. However, qubits have limited connectivity in existing QA hardware. This has spurred work on preprocessing algorithms for embedding the graph representing problem variables with quadratic terms into the hardware graph representing qubits adjacencies, such as the Chimera graph in hardware produced by D-Wave Systems. In this paper, we use integer linear programming to search for an embedding of the problem graph into certain classes of minors of the Chimera graph, which we call template embeddings. One of these classes corresponds to complete bipartite graphs, for which we show the limitation of the existing approach based on minimum odd cycle transversals (OCTs). One of the formulations presented is exact and thus can be used to certify the absence of a minor embedding using that template. On an extensive test set consisting of random graphs from five different classes of varying size and sparsity, we can embed more graphs than a state-of-the-art OCT-based approach, our approach scales better with the hardware size, and the runtime is generally orders of magnitude smaller.Summary of Contribution: Our work combines classical and quantum computing for operations research by showing that integer linear programming can be successfully used as a preprocessing step for adiabatic quantum optimization. We use it to determine how a quadratic unconstrained binary optimization problem can be solved by a quantum annealer in which the qubits are coupled as in a Chimera graph, such as in the quantum annealers currently produced by D-Wave Systems. The paper also provides a timely introduction to adiabatic quantum computing and related work on minor embeddings. }
}

@Article{Date2019,
author={Date, Prasanna
and Patton, Robert
and Schuman, Catherine
and Potok, Thomas},
title={Efficiently embedding QUBO problems on adiabatic quantum computers},
journal={Quantum Information Processing},
year={2019},
month={Mar},
day={05},
volume={18},
number={4},
pages={117},
abstract={Adiabatic quantum computers like the D-Wave 2000Q can approximately solve the QUBO problem, which is an NP-hard problem, and have been shown to outperform classical computers on several instances. Solving the QUBO problem literally means solving virtually any NP-hard problem like the traveling salesman problem, airline scheduling problem, protein folding problem, genotype imputation problem, thereby enabling significant scientific progress, and potentially saving millions/billions of dollars in logistics, airlines, healthcare and many other industries. However, before QUBO problems are solved on quantum computers, they must be embedded (or compiled) onto the hardware of quantum computers, which in itself is a very hard problem. In this work, we propose an efficient embedding algorithm, that lets us embed QUBO problems fast, uses less qubits and gets the objective function value close to the global minimum value. We then compare the performance of our embedding algorithm to that of D-Wave's embedding algorithm, which is the current state of the art, and show that our embedding algorithm convincingly outperforms D-Wave's embedding algorithm. Our embedding approach works with perfect Chimera graphs, i.e., Chimera graphs with no missing qubits.},
issn={1573-1332},
doi={10.1007/s11128-019-2236-3},
url={https://doi.org/10.1007/s11128-019-2236-3}
}

@Article{Sugie2021,
author={Sugie, and et al},
title={Minor-embedding heuristics for large-scale annealing processors with sparse hardware graphs of up to 102,400 nodes},
journal={Soft Computing},
year={2021},
month={Feb},
day={01},
volume={25},
number={3},
pages={1731-1749},
abstract={Minor-embedding heuristics have become an indispensable tool for compiling problems in quadratically unconstrained binary optimization (QUBO) into the hardware graphs of quantum and CMOS annealing processors. While recent embedding heuristics have been developed for annealers of moderate size (about 2000 nodes), the size of the latest CMOS annealing processor (with 102,400 nodes) poses entirely new demands on the embedding heuristic. This raises the question, if recent embedding heuristics can maintain meaningful embedding performance on hardware graphs of increasing size. Here, we develop an improved version of the probabilistic-swap-shift-annealing (PSSA) embedding heuristic [which has recently been demonstrated to outperform the standard embedding heuristic by D-Wave Systems (Cai et al. in http://arxiv.org/abs/1406.2741, 2014)] and evaluate its embedding performance on hardware graphs of increasing size. For random cubic and Bar{\'a}basi--Albert graphs we find the embedding performance of improved PSSA to consistently exceed the threshold of the best known complete graph embedding by a factor of 3.2 and 2.8, respectively, up to hardware graphs with 102,400 nodes. On the other hand, for random graphs with constant edge density not even improved PSSA can overcome the deterministic threshold guaranteed by the existence of the best known complete graph embedding. Finally, we prove a new upper bound on the maximal embeddable size of complete graphs into hardware graphs of CMOS annealers and show that the embedding performance of its currently best known complete graph embedding has optimal order for hardware graphs with fixed coordination number.},
issn={1433-7479},
doi={10.1007/s00500-020-05502-6},
url={https://doi.org/10.1007/s00500-020-05502-6}
}

@misc{dwaveQPU,
  author = {DWave Quantum Inc},
  title = {{The Most Connected and Powerful Quantum Computer Built for Business}},
  howpublished = "\url{https://www.dwavesys.com/solutions-and-products/systems/}",
  year = {2022},
}

@InProceedings{Zbinden2020,
author="Zbinden, Stefanie
and B{\"a}rtschi, Andreas
and Djidjev, Hristo
and Eidenbenz, Stephan",
title="Embedding Algorithms for Quantum Annealers with Chimera and Pegasus Connection Topologies",
booktitle="High Performance Computing",
year="2020",
address="Cham",
pages="187--206",
abstract="We propose two new algorithms -- Spring-Based MinorMiner (SPMM) and Clique-Based MinorMiner (CLMM) -- which take as input the connectivity graph of a Quadratic Unconstrained Binary Optimization (QUBO) problem and produce as output an embedding of the input graph on a host graph that models the topology of a quantum computing device. As host graphs, we take the Chimera graph and the Pegasus graph, which are the topology graphs of D-Wave's 2000 qubit (first introduced in 2017) and 5000 qubit (expected 2020) quantum annealer devices, respectively. We evaluate our algorithms on a large set of random graph QUBO inputs (Erd{\H{o}}s-R{\'e}nyi {\$}{\$}G{\_}{\{}n,p{\}}{\$}{\$}, Barab{\'a}si-Albert and d-regular graphs) on both host topologies against other embedding algorithms. For the Pegasus topology, we find that CLMM outperforms all other algorithms at edge densities larger than 0.08, while SPMM wins at edge densities smaller than 0.08 for Erd{\H{o}}s-R{\'e}nyi graphs, with very similar transition densities for the other graph classes. Surprisingly, the standard D-Wave MinorMiner embedding algorithm -- while also getting slightly outperformed by SPMM for sparse and very dense graphs on Chimera -- does not manage to extend its overall good performance on Chimera to Pegasus as it fails to embed even medium-density graphs on 175--180 nodes which are known to have clique embeddings on Pegasus.",
isbn="978-3-030-50743-5"
}

@InProceedings{Pinilla2019,
author="Pinilla, Jose P.
and Wilton, Steven J. E.",
title="Layout-Aware Embedding for Quantum Annealing Processors",
booktitle="High Performance Computing",
year="2019",
publisher="Springer International Publishing",
pages="121--139",
abstract="Due to the physical limit in connectivity between qubits in Quantum Annealing Processors (QAPs), when sampling from a problem formulated as an Ising graph model, it is necessary to embed the problem onto the physical lattice of qubits. A valid mapping of the problem nodes into qubits often requires qubit chains to ensure connectivity.",
isbn="978-3-030-20656-7"
}

@InProceedings{Sugie2018,
author="Sugie, and et al",
editor="Fagan, David
and Mart{\'i}n-Vide, Carlos
and O'Neill, Michael
and Vega-Rodr{\'i}guez, Miguel A.",
title="Graph Minors from Simulated Annealing for Annealing Machines with Sparse Connectivity",
booktitle="Theory and Practice of Natural Computing",
year="2018",
publisher="Springer International Publishing",
address="Cham",
pages="111--123",
abstract="The emergence of new annealing hardware in the last decade and its potential for efficiently solving NP hard problems in quadratically unconstrained binary optimization (QUBO) by emulating the ground state search of an Ising model are likely to become an important paradigm in natural computing. Driven by the need to parsimoniously exploit the limited hardware resources of present day and near-term annealers, we present a heuristic for constructing graph minors by means of simulated annealing. We demonstrate that our algorithm improves on state of the art hardware embeddings, allowing for the representation of certain QUBO problems with up to 50{\%} more binary variables.",
isbn="978-3-030-04070-3"
}

@misc{Marina2021,
  doi = {10.48550/ARXIV.2112.08300},
  
  url = {https://arxiv.org/abs/2112.08300},
  
  author = {Fernández-Campoamor, Marina and O'Meara, Corey and Cortiana, Giorgio and Peric, Vedran and Bernabé-Moreno, Juan},
  
  keywords = {Quantum Physics (quant-ph), Emerging Technologies (cs.ET), FOS: Physical sciences, FOS: Physical sciences, FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Community Detection in Electrical Grids Using Quantum Annealing},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {Creative Commons Attribution 4.0 International}
}

@article{Dillion2022,
    author = {Fox, Dillion M. AND MacDermaid, Christopher M. AND Schreij, Andrea M. A. AND Zwierzyna, Magdalena AND Walker, Ross C.},
    journal = {PLOS Computational Biology},
    publisher = {Public Library of Science},
    title = {{RNA} folding using quantum computers},
    year = {2022},
    month = {04},
    volume = {18},
    pages = {1-17},
    number = {4},

}

@Article{Charkiewicz2022,
author={Naecz-Charkiewicz, Katarzyna
and Nowak, Robert M.},
title={Algorithm for DNA sequence assembly by quantum annealing},
journal={BMC Bioinformatics},
year={2022},
month={Apr},
day={07},
volume={23},
number={1},
pages={122}
}


@ARTICLE{Neukart2017,
  
AUTHOR={Neukart and et al},   
	 
TITLE={Traffic Flow Optimization Using a Quantum Annealer},      
	
JOURNAL={Frontiers in ICT},      
	
VOLUME={4},           
	
YEAR={2017},      
	  
URL={https://www.frontiersin.org/articles/10.3389/fict.2017.00029},       
	
DOI={10.3389/fict.2017.00029},      
	
ISSN={2297-198X},   
   
ABSTRACT={Quantum annealing algorithms belong to the class of metaheuristic tools, applicable for solving binary optimization problems. Hardware implementations of quantum annealing, such as the quantum processing units (QPUs) produced by D-Wave Systems, have been subject to multiple analyses in research, with the aim of characterizing the technology’s usefulness for optimization and sampling tasks. In this paper, we present a real-world application that uses quantum technologies. Specifically, we show how to map certain parts of a real-world traffic flow optimization problem to be suitable for quantum annealing. We show that time-critical optimization tasks, such as continuous redistribution of position data for cars in dense road networks, are suitable candidates for quantum computing. Due to the limited size and connectivity of current-generation D-Wave QPUs, we use a hybrid quantum and classical approach to solve the traffic flow problem.}
}

@Article{Arute2019,
author={Arute, and et al,},
title={Quantum supremacy using a programmable superconducting processor},
journal={Nature},
year={2019},
month={Oct},
day={01},
volume={574},
number={7779},
pages={505-510},
abstract={The promise of quantum computers is that certain computational tasks might be executed exponentially faster on a quantum processor than on a classical processor1. A fundamental challenge is to build a high-fidelity processor capable of running quantum algorithms in an exponentially large computational space. Here we report the use of a processor with programmable superconducting qubits2--7 to create quantum states on 53 qubits, corresponding to a computational state-space of dimension 253 (about 1016). Measurements from repeated experiments sample the resulting probability distribution, which we verify using classical simulations. Our Sycamore processor takes about 200 seconds to sample one instance of a quantum circuit a million times---our benchmarks currently indicate that the equivalent task for a state-of-the-art classical supercomputer would take approximately 10,000 years. This dramatic increase in speed compared to all known classical algorithms is an experimental realization of quantum supremacy8--14 for this specific computational task, heralding a much-anticipated computing paradigm.},
issn={1476-4687},
doi={10.1038/s41586-019-1666-5},
url={https://doi.org/10.1038/s41586-019-1666-5}
}

@article{Shor1997,
author = {Shor, Peter W.},
title = {Polynomial-Time Algorithms for Prime Factorization and Discrete Logarithms on a Quantum Computer},
year = {1997},
issue_date = {Oct. 1997},
publisher = {Society for Industrial and Applied Mathematics},
address = {USA},
volume = {26},
number = {5},
issn = {0097-5397},
url = {https://doi.org/10.1137/S0097539795293172},
doi = {10.1137/S0097539795293172},
abstract = {A digital computer is generally believed to be an efficient universal computing device; that is, it is believed able to simulate any physical computing device with an increase in computation time by at most a polynomial factor. This may not be true when quantum mechanics is taken into consideration. This paper considers factoring integers and finding discrete logarithms, two problems which are generally thought to be hard on a classical computer and which have been used as the basis of several proposed cryptosystems. Efficient randomized algorithms are given for these two problems on a hypothetical quantum computer. These algorithms take a number of steps polynomial in the input size, e.g., the number of digits of the integer to be factored.},
journal = {SIAM J. Comput.},
pages = {1484–1509},
numpages = {26},
keywords = {spin systems, Fourier transforms, discrete logarithms, foundations of quantum mechanics, quantum computers, prime factorization, Church's thesis, algorithmic number theory}
}

@article{Ahmed2021,
title = {Quantum-Inspired Blockchain-Based Cybersecurity: Securing Smart Edge Utilities in IoT-Based Smart Cities},
journal = {Information Processing \& Management},
volume = {58},
number = {4},
pages = {102549},
year = {2021},
author = {Ahmed A. {Abd El-Latif} and et al},
keywords = {Blockchain, IoT, Smart City, Cybersecurity, Authentication, Encryption, Quantum Computation, Quantum-inspired, Quantum walks},
abstract = {Blockchain plays a vital task in cybersecurity. With the exerted efforts for realising large-scale quantum computers, most current cryptographic mechanisms may be hacked. Accordingly, we need a quantum tool utilised for designing blockchain frameworks to have the ability to be executed in the level of digital computers and resist the probable attacks from both digital and quantum computers. Quantum walks may be utilised as a quantum-inspired model for designing new cryptographic algorithms. In this paper, we present a new authentication and encryption protocol based on quantum-inspired quantum walks (QIQW). The proposed protocol is utilized to build a blockchain framework for secure data transmission among IoT devices. Instead of using classical cryptographic hash functions, quantum hash functions based on QIQW are employed for linking blocks of the chain. The main advantages of the presented framework are helping IoT nodes to effectively share their data with other nodes and full control of their records. Security analysis demonstrates that our proposed protocol can defend against message attack and impersonation attacks, thus ensuring secure transmission of data among IoT devices.}
}

@inproceedings{Jerbi2021,
 author = {Jerbi and et al},
 booktitle = {Advances in Neural Information Processing Systems},
 pages = {28362--28375},
 title = {Parametrized Quantum Policies for Reinforcement Learning},
 volume = {34},
 year = {2021}
}

@inproceedings{Bausch2020,
 author = {Bausch, Johannes},
 booktitle = {Advances in Neural Information Processing Systems},
 pages = {1368--1379},
 title = {Recurrent Quantum Neural Networks},
 url = {https://proceedings.neurips.cc/paper/2020/file/0ec96be397dd6d3cf2fecb4a2d627c1c-Paper.pdf},
 volume = {33},
 year = {2020}
}

@article{Akshay2019,
title = {Quantum computing for energy systems optimization: Challenges and opportunities},
journal = {Energy},
volume = {179},
pages = {76-89},
year = {2019},
issn = {0360-5442},
doi = {https://doi.org/10.1016/j.energy.2019.04.186},
url = {https://www.sciencedirect.com/science/article/pii/S0360544219308254},
author = {Akshay Ajagekar and Fengqi You},
keywords = {Quantum computing, Energy systems, Optimization},
abstract = {The purpose of this paper is to explore the applications of quantum computing to energy systems optimization problems and discuss some of the challenges faced by quantum computers with techniques to overcome them. The basic concepts underlying quantum computation and their distinctive characteristics in comparison to their classical counterparts are also discussed. Along with different hardware architecture description of two commercially available quantum systems, an example making use of open-source software tools is provided as a first step for diving into the new realm of programming quantum computers for solving systems optimization problems. The trade-off between qualities of these two quantum architectures is also discussed. Complex nature of energy systems due to their structure and large number of design and operational constraints make energy systems optimization a hard problem for most available algorithms. Problems like facility location allocation for energy systems infrastructure development, unit commitment of electric power systems operations, and heat exchanger network synthesis which fall under the category of energy systems optimization are solved using both classical algorithms implemented on conventional CPU based computer and quantum algorithm realized on quantum computing hardware. Their designs, implementation and results are stated. Additionally, this paper describes the limitations of state-of-the-art quantum computers and their great potential to impact the field of energy systems optimization.}
}

@misc{Farhi2014,
  doi = {10.48550/ARXIV.1411.4028},
  
  url = {https://arxiv.org/abs/1411.4028},
  
  author = {Farhi, Edward and Goldstone, Jeffrey and Gutmann, Sam},
  
  keywords = {Quantum Physics (quant-ph), FOS: Physical sciences, FOS: Physical sciences},
  
  title = {A Quantum Approximate Optimization Algorithm},
  
  publisher = {arXiv},
  
  year = {2014},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@Inbook{Bundy1984,
author="Bundy, Alan
and Wallen, Lincoln",
editor="Bundy, Alan
and Wallen, Lincoln",
title="Breadth-First Search",
bookTitle="Catalogue of Artificial Intelligence Tools",
year="1984",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="13--13",
abstract="An uninformed graph searching strategy in which each level is searched before going to the next deeper level. This strategy guarantees finding the shortest path to the node sought first: any path to the solution that is of length n will be found when the search reaches depth n, and this is guaranteed to be before any node of depth < n is searched.",
isbn="978-3-642-96868-6",
doi="10.1007/978-3-642-96868-6_25",
url="https://doi.org/10.1007/978-3-642-96868-6_25"
}

@misc{DWave_product,
  title = {The Most Connected and Powerful Quantum Computer Built for Business},
  howpublished = {\url{https://www.dwavesys.com/solutions-and-products/systems/}},
}

@misc{DWave_QA,
  title = {What is Quantum Annealing?},
  howpublished = {\url{https://docs.dwavesys.com/docs/latest/c_gs_2.html}},
}

@misc{DWave_topo,
  title = {What is Quantum Annealing?},
  howpublished = {\url{https://docs.dwavesys.com/docs/latest/c_gs_4.html}},
}

@article{Yarkoni2022,
author = {Yarkoni, Sheir and Raponi, Elena and Bäck, Thomas and Schmitt, Sebastian},
year = {2022},
month = {08},
pages = {},
title = {Quantum Annealing for Industry Applications: Introduction and Review},
volume = {85},
journal = {Reports on Progress in Physics},
doi = {10.1088/1361-6633/ac8c54}
}

@article{Finnila1994,
title = {Quantum annealing: A new method for minimizing multidimensional functions},
journal = {Chemical Physics Letters},
volume = {219},
number = {5},
pages = {343-348},
year = {1994},
author = {A.B. Finnila and M.A. Gomez and C. Sebenik and C. Stenson and J.D. Doll},
abstract = {Quantum annealing is a new method for finding extrema of multidimensional functions. Based on an extension of classical, simulated annealing, this approach appears robust with respect to avoiding local minima. Further, unlike some of its predecessors, it does not require an approximation to a wavefunction. We apply the technique to the problem of finding the lowest energy configurations of Lennard-Jones clusters of up to 19 particles (roughly 105 local minima). This early success suggests that this method may complement the widely implemented technique of simulated annealing.}
}

@ARTICLE{Lucas2014,
  
AUTHOR={Lucas, Andrew},   
	 
TITLE={Ising formulations of many NP problems},      
	
JOURNAL={Frontiers in Physics},      
	
VOLUME={2},           
	
YEAR={2014}
}

@misc{Boothby2020,
  doi = {10.48550/ARXIV.2003.00133},
  
  url = {https://arxiv.org/abs/2003.00133},
  
  author = {Boothby, Kelly and Bunyk, Paul and Raymond, Jack and Roy, Aidan},
  
  keywords = {Quantum Physics (quant-ph), FOS: Physical sciences, FOS: Physical sciences},
  
  title = {Next-Generation Topology of D-Wave Quantum Processors},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{DunningEtAl2018,
  title={What Works Best When? A Systematic Evaluation of Heuristics for Max-Cut and {QUBO}},
  author={Dunning, Iain and Gupta, Swati and Silberholz, John},
  year={2018},
  journal={{INFORMS} Journal on Computing},
  volume={30},
  number={3}
}

@article{Culberson1995,
  title={Hiding our colors},
  author={J. Culberson, A. Beacham, and D. Papp},
  year={1995},
  journal={CP’95 Workshop on Studying and Solving Really Hard Problems},
}

@article{Beasley1990,
 ISSN = {01605682, 14769360},
 URL = {http://www.jstor.org/stable/2582903},
 abstract = {In this note we present a system (OR-Library) that distributes test problems by electronic mail (e-mail). This system currently has available test problems drawn from a number of different areas of operational research.},
 author = {J. E. Beasley},
 journal = {The Journal of the Operational Research Society},
 number = {11},
 pages = {1069--1072},
 publisher = {Palgrave Macmillan Journals},
 title = {OR-Library: Distributing Test Problems by Electronic Mail},
 urldate = {2022-10-28},
 volume = {41},
 year = {1990}
}

@ARTICLE{Guillaume2022,
  author={Guillaume and et al},
  journal={IEEE Transactions on Quantum Engineering}, 
  title={Deep Space Network Scheduling Using Quantum Annealing}, 
  year={2022},
  volume={3},
  number={},
  pages={1-13},
  doi={10.1109/TQE.2022.3199267}}

@Article{Ding2021,
author={Ding and et al},
title={Implementation of a Hybrid Classical-Quantum Annealing Algorithm for Logistic Network Design},
journal={SN Computer Science},
year={2021},
month={Feb},
day={02},
volume={2},
number={2},
pages={68},
abstract={The logistic network design is an abstract optimization problem that, under the assumption of minimal cost, seeks the optimal configuration of the supply chain's infrastructures and facilities based on customer demand. Key economic decisions are taken about the location, number, and size of manufacturing facilities and warehouses based on the optimal solution. Therefore, improvements in the methods to address this question, which is known to be in the NP-hard complexity class, would have relevant financial consequences. Here, we implement in the D-Wave quantum annealer a hybrid classical-quantum annealing algorithm. The cost function with constraints is translated to a spin Hamiltonian, whose ground state encodes the searched result. As a benchmark, we measure the accuracy of results for a set of paradigmatic problems against the optimal published solutions (the error is on average below {\$}{\$}1{\backslash}{\%}{\$}{\$}), and the performance is compared against the classical algorithm, showing a remarkable reduction in the number of iterations. This work shows that state-of-the-art quantum annealers may codify and solve relevant supply-chain problems even still far from useful quantum supremacy.},
issn={2661-8907},
doi={10.1007/s42979-021-00466-2},
url={https://doi.org/10.1007/s42979-021-00466-2}
}

@INPROCEEDINGS{Ishizaki2019,
  author={Ishizaki, Fumio},
  booktitle={2019 13th International Conference on Signal Processing and Communication Systems (ICSPCS)}, 
  title={Computational Method Using Quantum Annealing for TDMA Scheduling Problem in Wireless Sensor Networks}, 
  year={2019},
  volume={},
  number={},
  pages={1-9},
  doi={10.1109/ICSPCS47537.2019.9008543}}

@book{Cohenbook2010,
author = {Cohen, J. and Powderly, William and Opal, S.M.},
year = {2010},
month = {01},
pages = {1-1918},
title = {Infectious Diseases: Third Edition},
journal = {Infectious Diseases: Third Edition}
}

@article{shankarappa2014,
author = {Sahadev A Shankarappa and et al},
title ={Efficacy versus Toxicity - The Ying and Yang in Translating Nanomedicines},
journal = {Nanomaterials and Nanotechnology},
volume = {4},
pages = {23},
year = {2014}
}

@Inbook{Riley2010,
author="Riley, Anthony L.
and Kohut, Steve",
editor="Stolerman, Ian P.",
title="Drug Toxicity",
bookTitle="Encyclopedia of Psychopharmacology",
year="2010",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="441--441"
}

@article{Robertson2007EnzymesAA,
  title={Enzymes as a special class of therapeutic target: clinical drugs and modes of action.},
  author={James G. Robertson},
  journal={Current opinion in structural biology},
  year={2007},
  volume={17 6},
  pages={        674-9    }
}

@article{Robertson2005MechanisticBO,
  title={Mechanistic basis of enzyme-targeted drugs.},
  author={James G. Robertson},
  journal={Biochemistry},
  year={2005},
  volume={44 15},
  pages={       5561-71}
}

@Article{medicina57111209,
AUTHOR = {Berillo, Dmitriy and Yeskendir, Adilkhan and Zharkinbekov, Zharylkasyn and Raziyeva, Kamila and Saparov, Arman},
TITLE = {Peptide-Based Drug Delivery Systems},
JOURNAL = {Medicina},
VOLUME = {57},
YEAR = {2021},
NUMBER = {11},
ARTICLE-NUMBER = {1209}
}

@ARTICLE{Mengqian2020,
AUTHOR={Li, Mengqian and Zhao, Guangkuo and Su, Wei-Ke and Shuai, Qi},   
TITLE={Enzyme-Responsive Nanoparticles for Anti-tumor Drug Delivery},      
JOURNAL={Frontiers in Chemistry},      
VOLUME={8},     	
YEAR={2020}
}

@ARTICLE{Martorana2014,
AUTHOR={Martorana, Alessandro and Koch, Giacomo},   
TITLE={“Is dopamine involved in Alzheimer's disease?”},      
JOURNAL={Frontiers in Aging Neuroscience},      
VOLUME={6},           
YEAR={2014}
}

@article{Pritchard2009,
title = "Investigation of dopamine receptors in susceptibility to behavioural and psychological symptoms in Alzheimer's disease",
author = "AL Pritchard and L Ratcliffe and E Sorour and Mohammad Haque and Roger Holder and Peter Bentham and CL Lendon",
year = "2009",
month = aug,
day = "14",
language = "English",
volume = "24",
pages = "1020--1025",
journal = "International Journal of Geriatric Psychiatry",
publisher = "Wiley",
number = "9",
}

@Article{ijms21041258,
AUTHOR = {D’Avanzo, Francesca and Rigon, Laura and Zanetti, Alessandra and Tomanin, Rosella},
TITLE = {Mucopolysaccharidosis Type II: One Hundred Years of Research, Diagnosis, and Treatment},
JOURNAL = {International Journal of Molecular Sciences},
VOLUME = {21},
YEAR = {2020},
NUMBER = {4}
}

@inbook{cooney2017,
author = {Cooney, Michael},
year = {2017},
month = {10},
pages = {215-232},
title = {Kinetic Measurements for Enzyme Immobilization},
volume = {1504},
journal = {Methods in molecular biology (Clifton, N.J.)}
}

@article{Terentis2010TheSD,
  title={The selenazal drug ebselen potently inhibits indoleamine 2,3-dioxygenase by targeting enzyme cysteine residues.},
  author={Andrew C Terentis and Mohammed Freewan and Tito S Semp{\'e}rtegui Plaza and Mark J. Raftery and Roland Stocker and S. R. Thomas},
  journal={Biochemistry},
  year={2010},
  volume={49 3},
  pages={591-600}
}

@article{Mizutani2012RelatingDI,
  title={Relating drug–protein interaction network with drug side effects},
  author={Sayaka Mizutani and Edouard Pauwels and V{\'e}ronique Stoven and Susumu Goto and Yoshihiro Yamanishi},
  journal={Bioinformatics},
  year={2012},
  volume={28},
  pages={i522 - i528}
}

@article{Copeland2007TargetingEI,
  title={Targeting enzyme inhibitors in drug discovery},
  author={Robert A Copeland and Mark R. Harpel and Peter J. Tummino},
  journal={Expert Opinion on Therapeutic Targets},
  year={2007},
  volume={11},
  pages={967 - 978}
}

@incollection{KAMBUR2010227,
title = {Catechol-O-Methyltransferase and Pain},
editor = {Erkki Nissinen},
series = {International Review of Neurobiology},
author = {Oleg Kambur and Pekka T. Mannisto},
publisher = {Academic Press},
volume = {95},
pages = {227-279},
year = {2010}
}

@article{BARSE200736,
title = {Endocrine disruption and metabolic changes following exposure of Cyprinus carpio to diethyl phthalate},
author = {A.V. Barse and T. Chakrabarti and T.K. Ghosh and A.K. Pal and S.B. Jadhao},
journal = {Pesticide Biochemistry and Physiology},
volume = {88},
number = {1},
pages = {36-42},
year = {2007}
}


@article{naylor1981,
title = {Urinary pyrimidine excretion in arginase deficiency},
author = {E. W. Naylor and S. D. Cederbaum},
volume = {4},
number = {1},
pages = {207-210},
year = {1981}
}

@article{Pandhare2009RegulationAF,
  title={Regulation and function of proline oxidase under nutrient stress},
  author={Jui Pandhare and Steven P. Donald and Sandra K. Cooper and James M. Phang},
  journal={Journal of Cellular Biochemistry},
  year={2009},
  volume={107}
}

@article{cruzat2018,
title = "Glutamine: Metabolism and immune function, supplementation and clinical translation",
keywords = "Amino acids, Gut, Leukocytes, Liver, Nutrition, Skeletal muscle",
author = "Vinicius Cruzat and Rogero, {Marcelo Macedo} and Keane, {Kevin Noel} and Rui Curi and Philip Newsholme",
year = "2018",
month = nov,
day = "1",
language = "English",
volume = "10",
journal = "Nutrients",
publisher = "Multidisciplinary Digital Publishing Institute (MDPI)",
number = "11",
}
